Multi-LLM Collaborative Search for Complex Problem Solving

Large language models (LLMs) often struggle with complex reasoning tasks due to their limitations in addressing the vast reasoning space and inherent ambiguities of natural language. We propose the Mixture-of-Search-Agents (MoSA) paradigm, a novel approach leveraging the collective expertise of multiple LLMs to enhance search-based reasoning. MoSA integrates diverse reasoning pathways by combining independent exploration with iterative refinement among LLMs, mitigating the limitations of single-model approaches. Using Monte Carlo Tree Search (MCTS) as a backbone, MoSA enables multiple agents to propose and aggregate reasoning steps, resulting in improved accuracy. Our comprehensive evaluation across four reasoning benchmarks demonstrates MoSA's consistent performance improvements over single-agent and other multi-agent baselines, particularly in complex mathematical and commonsense reasoning tasks.

==> algorithms/general_mcts.tex <==
% \begin{figure*}[t]
% \begin{center}
% \scalebox{1.0}{
% \begin{minipage}{0.7\textwidth}
% \begin{algorithm}[H]
% \caption{Expansion Step in MCTS}
% \label{alg:expand}
% \begin{algorithmic}
% \REQUIRE Current node $s_i$, Generator policy $\pi^*$
% \ENSURE Expanded nodes added to the tree

% \STATE Initialize empty list $\texttt{\small expanded\_nodes}$
% \STATE Let \hspace{1pt} $\texttt{\small parent\_node} \leftarrow s_i$
% \STATE Let \hspace{1pt} $\texttt{\small p\_state} \leftarrow \texttt{\small parent\_node.state}$

% \STATE \COMMENTALGO{Generate actions from the current state}
% \FOR{each $\texttt{\small action} \in \texttt{\small GenerateActions}(\texttt{\small p\_state})$}
%     \STATE \COMMENTALGO{Compute transition using concatenation}
%     \STATE $\texttt{\small new\_state} \leftarrow \mathtt{concat}(\texttt{\small p\_state},\hspace{2pt} \texttt{\small action})$

%     \STATE \COMMENTALGO{Create a new child node}
%     \STATE $\texttt{\small child\_node} \leftarrow \texttt{\small Node}(\texttt{\small state=new\_state},\hspace{2pt} \texttt{\small parent=parent\_node})$
    
%     \STATE \COMMENTALGO{Add the child node to the search tree}
%     \STATE $\texttt{\small AddChild}(\texttt{\small parent\_node},\hspace{2pt} \texttt{\small child\_node})$
    
%     \STATE \COMMENTALGO{Store the expanded node}
%     \STATE $\texttt{\small expanded\_nodes.append}(\texttt{\small child\_node})$
% \ENDFOR

% \STATE \textbf{return} $\texttt{\small expanded\_nodes}$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% }
% \end{center}
% \end{figure*}


\begin{algorithm}[tb]
\caption{\emph{Expansion} step in MCTS. This work focuses on the \texttt{GenerateActions} function, which is illustrated in Algorithm~\ref{alg:mosa-A_1} in more details.}
\label{alg:expand}
\begin{algorithmic}
\REQUIRE Selected node $s_i$, Generator policy $\pi^*$
\ENSURE Expanded nodes added to the tree

\STATE Initialize empty list $\texttt{\small expanded\_nodes}$
\STATE Let \hspace{1pt} $\texttt{\small parent\_node} \leftarrow s_i$
\STATE Let \hspace{1pt} $\texttt{\small p\_state} \leftarrow \texttt{\small parent\_node.state}$

% \STATE Let $\texttt{\small curr\_actions} \leftarrow \texttt{\small GenerateActions}(\texttt{\small p\_state})$
\STATE \COMMENTALGO{Generate actions from the current state}
\FOR{each $\texttt{\small action} \in \texttt{\small GenerateActions}(\texttt{\small p\_state})$}
    \STATE \COMMENTALGO{State transition as concatenation}
    \STATE $\texttt{\small new\_state} \leftarrow \texttt{\small concat}(\texttt{\small p\_state},\hspace{2pt} \texttt{\small action})$

    \STATE \COMMENTALGO{Create a new child node}
    \STATE $\texttt{\small child\_node} \leftarrow \texttt{\small Node}(\texttt{\small state=new\_state},\hspace{2pt} \texttt{\small parent}$
    \STATE $\texttt{\small =parent\_node})$
    
    \STATE \COMMENTALGO{Add the child node to the search tree}
    \STATE $\texttt{\small AddChild}(\texttt{\small parent\_node},\hspace{2pt} \texttt{\small child\_node})$
    
    \STATE \COMMENTALGO{Store the expanded node}
    \STATE $\texttt{\small expanded\_nodes.append}(\texttt{\small child\_node})$
\ENDFOR

\STATE \textbf{return} $\texttt{\small expanded\_nodes}$
\end{algorithmic}
\end{algorithm}

==> algorithms/generate_action_vanilla.tex <==
\begin{algorithm}[tb]
\caption{\texttt{\small GenerateActions} {\small with a single LLM}}
\label{alg:expand}
\begin{algorithmic}
\REQUIRE Selected node $s$, LLM $\pi$, number of sub-questions $n_1$, number of sub-answers per sub-question $n_2$, sampling hyper-parameters for LLM generation $\theta$
\ENSURE Generate a set of new actions $\{a_1, a_2, ..., a_{n_1}\}$

\STATE Initialize empty list $\texttt{\small new\_actions}$
\STATE Let \hspace{1pt} $\texttt{\small parent\_node} \leftarrow s$
\STATE Let \hspace{1pt} $\texttt{\small p\_state} \leftarrow \texttt{\small parent\_node.state}$

\FOR{$i=1$ {\bfseries to} $n_1$}
% \STATE Let $\texttt{\small curr\_actions} \leftarrow \texttt{\small GenerateActions}(\texttt{\small p\_state})$
\STATE \COMMENTALGO{Sample the next sub-question given $s$}
\STATE $\texttt{\small sub\_q}_i \leftarrow \pi(\cdot|s)$

\STATE Initialize an empty list for candidate sub-answers $\texttt{\small cand\_ans}$
\FOR{$i=1$ {\bfseries to} $n_2$}
\STATE \COMMENTALGO{Sample the next sub-answer given $\texttt{\small concat(} s \texttt{\small, sub\_q}_i \texttt{\small )} $}
\STATE $\texttt{\small sub\_a}_{ij} \leftarrow \pi(\cdot|\texttt{\small concat(} s \texttt{\small, sub\_q}_i \texttt{\small )})$
\STATE \COMMENTALGO{Store the candidate sub-answer}
\STATE $\texttt{\small cand\_ans.append(sub\_a}_{ij} \texttt{\small )}$
\ENDFOR

\ENDFOR

\STATE \textbf{return} $\texttt{\small expanded\_nodes}$
\end{algorithmic}
\end{algorithm}

==> tables/exp-abstraction.tex <==
\begin{table*}[t]
\caption{
Abstractions of various approaches. Under similar hyperparameter settings, we have $n_1 < n_2 < p n_1$ and $n_3 > n_2$, where $1 < p < 2$. As the number of proposed sub-answers increases, $n_1$ would increases and $p$ will decreases. In other words, with larger numbers of returning sequences in \textsc{MoSA}, the computational overhead introduced by aggregators becomes smaller.
}
\label{tab:abstraction}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccc}
\toprule
Method & Action Space & \# Proposers & \# Aggregators & \# Forward Calls \\
\midrule
Few-shot CoT & $A2$ & Single & None & 1 \\
Self-Consistency@$n$ (\emph{w/} a single LLM) & $A2$ & Single & None & $n$ \\
Self-Consistency@$n$ (\emph{w/} all LLMs) & $A2$ & Multi & None & $n$ \\
RAP (\emph{w/o} aggregators) & $A\{2,3\}$ & Single & None & $n_1$ \\
RAP (\emph{w/} aggregators) & $A\{2,3\}$ & Single & Single & $n_2$ \\
\ourmethod{} (\emph{w/o} aggregators) & $A\{2,3\}$ & Multi & None & $n_1$ \\
\ourmethod{} (\emph{w/} aggregators) & $A\{2,3\}$ & Multi & Multi & $n_2$ \\
rStar (majority voting) & $A\{1,2,3,4,5\}$ & Single & None & $n_3$ \\
rStar (majority voting) + \ourmethod{} (\emph{w/o} aggregators) & $A\{1,2,3,4,5\}$ & Multi & None & $n_3$ \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


==> tables/exp-moa.tex <==
\begin{table*}[t]
\caption{
The results of Mixture-of-Agents (MoA, \citet{moa}). MoA can be seen as a specific case of \textsc{MoSA}.
MoA's only available action is to directly propose the final answer; thus, there is no search in MoA.
The accuracy gaps between MoA (depth=5) and \ourmethod{} suggest that search is critical to reasoning performances.
}
\label{tab:moa}
\vskip 0.15in
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{lcccc}
\toprule
Method & GSM8K & SVAMP & MATH & StrategyQA \\
\midrule
MoA (depth=1) & 90.67 & 93.40 & 52.60 & 71.62 \\
MoA (depth=5) & 90.67 &  &  & 70.60 \\
\ourmethod{} &  \textbf{91.96} &  \textbf{94.90} &  \textbf{56.60} &  \textbf{77.73}  \\
\bottomrule
\end{tabular}
% \end{sc}
% \end{small}
\end{center}
\vskip -0.1in
\end{table*}


==> tables/exp-num_of_agents.tex <==
\begin{table}[t]
\caption{
Number of distinct search agents.
}
\label{tab:num_of_agents}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{ccccc}
\toprule
\#Agents & GSM8K & SVAMP & MATH & StrategyQA \\
\midrule
1 & 90.05  & 92.50 & 54.80 & 75.69 \\
2 & 91.13  & 93.30 & 55.65 & 76.56 \\
3 & 91.81  & 94.40 & \textbf{56.85} & 77.58  \\
4 &  \textbf{91.96} &  \textbf{94.90} &  56.60 &  \textbf{77.73} \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
